Enhanced pedestal transport driven by edge collisionality on Alcator C-Mod and its role in regulating H-mode pedestal gradients

Experimental measurements of plasma and neutral profiles across the pedestal are used in conjunction with 2D edge modeling to examine pedestal stiffness in Alcator C-Mod H-mode plasmas. Experiments on Alcator C-Mod observed pedestal degradation and loss in confinement below a critical value of net power crossing the separatrix, $P_\mathrm{net} = P_\mathrm{net}^\mathrm{crit} \approx 2.3$ MW. New analysis of ionization and particle flux profiles reveal saturation of the pedestal electron density, $n_{e}^\mathrm{ped}$ despite continuous increases in ionization throughout the pedestal, inversely related to $P_\mathrm{net}$. A limit to the pedestal $\nabla n_{e}$ emerges as the particle flux, $\Gamma_{D}$ continues to grow, implying increases in the effective particle diffusivity, $D_\mathrm{eff}$. This is well-correlated with the separatrix collisionality, $\nu^{*}_\mathrm{sep}$ and a turbulence control parameter, $\alpha_{t}$, implying a possible transition in type of turbulence. The transition is well correlated with the experimentally observed value of $P_\mathrm{net}^\mathrm{crit}$. SOLPS-ITER modeling is performed for select discharges from the power scan, constrained with experimental electron and neutral densities, measured at the outer midplane. The modeling confirms general growth in $D_\mathrm{eff}$, consistent with experimental findings, and additionally suggests even larger growth in $\chi_{e}$ at the same $P_\mathrm{net}^\mathrm{crit}$.

==> outline.tex <==
\label{sec:outline}

\begin{enumerate}
    \item Background
    \begin{enumerate}
        \item Predicting density pedestal
        \item Importance of source for prediction
        \item C-Mod opaqueness
        \item Transport-limited pedestals
    \end{enumerate}
    \item Database building and sub-selection
    \begin{enumerate}
        \item Lyman-alpha camera
        \item Edge Thomson scattering 
        \item Computing other neutral quantities
        \item Sub-select to fixed field and current
    \end{enumerate}
    \item Pedestal stiffness
    \begin{enumerate}
        \item $n_{e}$ vs $S_{ion}$ at pedestal - maybe also at separatrix? look at wall pressure as well?
        \item Flux-gradient at different positions of the pedestal - spans range of transport - rapid growth of inferred transport
        \item Show $D_{eff}$ profiles - consider $v_{eff}$ as well?
        \item Compare penetration lengths with pedestal widths?
    \end{enumerate}
    \item Fluctuation measurements and correlation with transport
    \begin{enumerate}
        \item PCI analysis and QCM identification
        \item Comparison of mode strength with  $D_{eff}$
        \item ***Worth looking into reflectometer?
        \item Changes at targets seem to track $P_{net}$ - does this deserve its own section?
    \end{enumerate}
    \item Pedestal operational space and hypothesis of collisionality driver
    \begin{enumerate}
        \item Density vs temperature - isobars and isocollisionality - *** shift in pedestal position as a source of decreased pressure gradient?
        \item Pedestal pressure and gradient with collisionality
        \item Changes to transport with collisionality at separatrix? ***introduce $\alpha_{t}$ - maybe also calculate some other turbulence parameters and look at relationships 
        \item *** Pressure gradient widening with $\alpha_{t}$? How does this work its way up to the pedestal? Turbulence spreading?
    \end{enumerate}
    \item SOLPS simulations
    \begin{enumerate}
        \item Procedure for matching $n_{e}$, $T_{e}$ using $D$, $\chi$
        \item Matching neutrals solution through modifying boundary conditions
        \item Analyze transport profile in pedestal
        \item Is there anything to add regarding poloidal variation? May need some more analysis here. Targets?
    \end{enumerate}
    \item ***Pumping and upper null plasmas
        \begin{enumerate}
        \item ***Replot $n_{e}$ vs. $S_{ion}$ including pumping
        \item ***Changes to $D_{eff}$ - what does the QCM do?
        \item ***Do we change turbulent transport regime? Recover drift-wave turbulence? Maybe try to look at $\eta_{e}$ again
        \item What happens in USN? How does pumping work there?
    \item ***Model for $D_{eff}$ with collisionality?
        \item Is there a way to implement this in SOLPS parametrically
        \item Anything related to $\eta_{e}$
    \end{enumerate}
    
\end{enumerate}
